Dynamics for Galactic Archaeology

Our Galaxy is a complex machine in which several processes operate simultaneously: metal-poor gas is accreted, is chemically enriched by dying stars, and then drifts inwards, surrendering its angular momentum to stars; new stars are formed on nearly circular orbits in the equatorial plane and then diffuse through orbit space to eccentric and inclined orbits; the central stellar bar surrenders angular momentum to the surrounding disc and dark halo while acquiring angular momentum from inspiralling gas; the outer parts of the disc are constantly disturbed by satellite objects, both luminous and dark, as they sweep through pericentre. We review the conceptual tools required to bring these complex happenings into focus. Our first concern must be the construction of equilibrium models of the Galaxy, for upon these hang our hopes of determining the Galaxy's mean gravitational field, which is required for every subsequent step. Ideally our equilibrium model should be formulated so that the secular evolution of the system can be modelled with perturbation theory. Such theory can be used to understand how stars diffuse through orbit space from either the thin gas disc in which we presume disc stars formed, or the debris of an accreted object, the presumed origin of many halo stars. Coupling this understanding to the still very uncertain predictions of the theory of stellar evolution and nucleosynthesis, we can finally extract a complete model of the chemodynamic evolution of our reasonably generic Galaxy. We discuss the relation of such a model to cosmological simulations of galaxy formation, which provide general guidance but cannot be relied on for quantitative detail.

==> binneymac.tex <==
\arraycolsep0.35mm                      % makes multiple equations look nice
\catcode`\@=11
\def\gta{\ifmmode{\,\mathrel{\mathpalette\@versim>\,}}
    \else{$\,\mathrel{\mathpalette\@versim>}\,$}\fi}
\def\lta{\ifmmode{\,\mathrel{\mathpalette\@versim<\,}}
    \else{$\,\mathrel{\mathpalette\@versim<}\,$}\fi}
\def\@versim#1#2{\lower 2.9truept \vbox{\baselineskip 0pt \lineskip
    0.5truept \ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
\catcode`\@=12  
%%%%%%%%%%%%%%%%%%%
% My own definitions
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}
\def\const{\hbox{constant}}
% Bold face Greek letters
%
\font\gkvecten=cmmib10
\font\gkvecseven=cmmib7
\let\boldgrk=\gkvecten
\let\boldgrksc=\gkvecseven

\def\gkthing#1{{\mathchoice%
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}}}
\def\rms{{\sc rms}}
\def\valpha{\gkthing{11}}
\def\vbeta{\gkthing{12}}
\def\vgamma{\gkthing{13}}
\def\vdelta{\gkthing{14}}
\def\vepsilon{\gkthing{15}}
\def\vzeta{\gkthing{16}}
\def\veta{\gkthing{17}}
\def\vtheta{\gkthing{18}}
\def\viotaeta{\gkthing{19}}
\def\vkappa{\gkthing{20}}
\def\vlambda{\gkthing{21}}
\def\vmu{\gkthing{22}}
\def\vnu{\gkthing{23}}
\def\vxi{\gkthing{24}}
\def\vpi{\gkthing{25}}
\def\vrho{\gkthing{26}}
\def\vsigma{\gkthing{27}}
\def\vtau{\gkthing{28}}
\def\vupsilon{\gkthing{29}}
\def\vphi{\gkthing{30}}
\def\vchi{\gkthing{31}}
\def\vpsi{\gkthing{32}}
\def\vomega{\gkthing{33}}
\def\vDelta{{\bf\Delta}}
\def\vOmega{{\bf\Omega}}
\def\Omegap{\Omega_{\rm p}}
\def\ket#1{|#1\rangle}\def\bra#1{\langle#1|}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname v\expandafter\top\veclist\endcsname%
{{\noexpand\bf\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZ.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname c\expandafter\top\veclist\endcsname%
{{\noexpand\cal\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
\def\i{{\rm i}}
\def\df{{\sc df}}\def\edf{{\sc edf}}
\def\dm{{\sc dm}}
\def\CR{{\sc cr}}\def\ILR{{\sc ilr}}\def\OLR{{\sc olr}}
\def\cE{{\cal E}}
\def\SN{S_{\rm N}}
\def\SNIa{SN$\,$Ia}
\def\Teff{T_{\rm eff}}
\def\logg{\log g}
\def\feh{[{\rm Fe/H}]}\def\afe{[\alpha/{\rm Fe}]}
\def\vlos{v_{\rm los}}
\def\fracj#1#2{{\textstyle{#1\over#2}}}
\def\deffn#1{{\bf#1}}
\def\pa{\partial}
\def\ex#1{\left\langle#1\right\rangle}
\def\Rc{R_{\rm c}}\def\vc{v_{\rm c}}
\def\Phic{\Phi_{\rm c}}
\def\Phieff{\Phi_{\rm eff}}
\def\cm{\,{\rm cm}}
\def\kms{\,{\rm km}\,{\rm s}^{-1}}
\def\mag{\,{\rm mag}}
\def\Myr{\,{\rm Myr}}
\def\yr{\,{\rm yr}}
\def\Gyr{\,{\rm Gyr}}
\def\K{\,{\rm K}} \let\kelvin=\K
\def\pc{\,{\rm pc}}
\def\kpc{\,{\rm kpc}}
\def\Mpc{\,{\rm Mpc}}
\def\ergs{\,{\rm erg}}
\def\hi{H\,{\sc i}}
\def\e{{\rm e}}
\def\d{{\rm d}}
\def\msun{\,{\rm M}_\odot}
\def\Fe{{\rm Fe}}
\def\meh{\hbox{[Me/H]}}
\def\feh{\hbox{[Fe/H]}}
\def\cafe{[\hbox{Ca}/\hbox{Fe}]}
\def\ofe{[\hbox{O}/\hbox{Fe}]}
\def\zeh{\hbox{[$Z$/H]}}
\def\alphaH{[\alpha/\hbox{H}]}
\def\afe{[\alpha/\hbox{Fe}]}
\def\dex{\,{\rm dex}}
\def\Rg{R_{\rm g}}
\def\vpbar{\overline{v}_\phi}
\def\figref#1{Fig.~\ref{#1}}
%%%%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

